Improving the Serving Performance of Multi-LoRA Large Language Models via Efficient LoRA and KV Cache Management

Multiple Low-Rank Adapters (Multi-LoRAs) are gaining popularity for task-specific Large Language Model (LLM) applications. For multi-LoRA serving, caching hot KV caches and LoRA adapters in high bandwidth memory of accelerations can improve inference performance. However, existing Multi-LoRA inference systems fail to optimize serving performance like Time-To-First-Toke (TTFT), neglecting usage dependencies when caching LoRAs and KVs. We therefore propose FASTLIBRA, a Multi-LoRA caching system to optimize the serving performance. FASTLIBRA comprises a dependency-aware cache manager and a performance-driven cache swapper. The cache manager maintains the usage dependencies between LoRAs and KV caches during the inference with a unified caching pool. The cache swapper determines the swap-in or out of LoRAs and KV caches based on a unified cost model, when the HBM is idle or busy, respectively. Experimental results show that ELORA reduces the TTFT by 63.4% on average, compared to state-of-the-art works.

==> Sections/evaluation.tex <==
\section{Evaluation of ELoRA\label{eval}}
In this section, we first show the serving performance of \sysname{} under various Multi-LoRA application scenarios.
% compared to the state-of-the-art Multi-LoRA inference systems. 
% we first show the serving performance of \sysname{} compared to the state-of-the-art Multi-LoRA inference systems. 
% The experiments are conducted according to various models and scenarios. 
Then, we dive into the reasons behind the performance gains achieved by \sysname{} and effectiveness of its individual modules. 
At last, we evaluate the stability of \sysname{} in a broader range of LoRA number and query distributions.

\subsection{Evaluation Setup}
% \SJC{Be concise.}
% \textbf{Draft, need modify}
% hardware+software, traces+dataset, baselines
% \textbf{Hardware.} 
% Our hardware configuration is based on the Atlas 800 training server with 8 high-performance Atlas 300I NPUs shown in Table~\ref{table:config}. 

Table~\ref{table:config} has shown our experimental platform.

\textbf{Model.} We used one of the most popular large model series, Llama, for testing. We selected various sizes of Llama models and chose suitable testing hardware devices based on the model size, as shown in Table~\ref{tab:model_setting}. Besides Llama, our system can also be easily adapted to any decoder-only transformer models, such as the GPT series.
In each experiment group, we selected an appropriate number of NPU computing cards and main memory size based on the model parameter size for inference.

\begin{table}[htbp]
    \centering
    \small
    \caption{Base models and settings}
    \begin{tabular}{c|c}
        \hline
        Base model & \textbf{Setting}  \\
        \hline
        Llama-7B & 1 High-performance NPU @ 64GB Main Memory  \\
        \hline
        Llama-13B & 2 High-performance NPU @ 128GB Main Memory   \\
        \hline
        Llama-34B & 4 High-performance NPU @ 256GB Main Memory  \\
        \hline
    \end{tabular}
    \label{tab:model_setting}
\end{table}

For LoRAs, following previous work~\cite{}, we constructed them based on the model parameters and set the rank of LoRAs to 32 and 64 uniformly. 
For each model, we constructed various numbers of LoRAs. 
The parameters of the LoRAs are randomly generated using a normal distribution. Since we always fixed the input and output lengths of the queries according to the dataset, this initialization does not affect the amount of calculation. 

\textbf{Baseline.} We select state-of-art Mult-LoRA inference system, vLLM and S-LoRA as baseline. 

% \textbf{vLLM.} vLLM is currently one of the best-performing large model inference systems with a significant number of code contributors and popularity in the open-source community, including many features like Multi-LoRA inferencing and prefix-cache.
% % Although the original version of vLLM did not consider Multi-LoRA inference and history KV caching, the latest open-source version of vLLM has implemented a Multi-LoRA inference and KV caching matching system.
% % As previously mentioned, vLLM statically manages memory allocation for LoRAs, requiring users to pre-determine the memory pool ratio allocated to LoRAs on HBM, which cannot be changed during running. Therefore, in dynamic scenarios, the optimal memory pool ratio is constantly changing. We set the memory pool ratio to 20% in our experimental group, which allows for the loading of exactly 20 different LoRAs.
% vLLM implements the KV caching matching system using a hash table. However, vLLM only uses HBM to store history KV caches and does not consider a swap-out mechanism for history KV caches. When HBM memory is insufficient, it directly evicts KV cache based on the LRU policy. To ensure a fair comparison, we also implemented the use of main memory for storing history KV caches in vLLM and realizing swap-out based on the LRU policy when HBM memory is insufficient and pre-fetching them back based on the LRU policy when HBM memory is sufficient.

% \textbf{S-LoRA.} S-LoRA implements batched Multi-LoRA inference and the unified memory pool for LoRAs and KV caches. However, it does not consider the reuse of history KV caches and directly abandons KV caches after queries finish. For LoRAs, S-LoRA follows the on-demand swapping principle, swapping in the required LoRAs during inference and swapping out the LoRAs after inferencing, to free up more HBM memory space for inference.

\begin{enumerate}
    \item \textbf{vLLM.} vLLM is a high-performing large model inference system widely used in the open-source community, with the latest capabilities like Multi-LoRA inference and prefix-cache. It uses a hash table to implement the KV cache matching system, storing history KV caches in HBM without a swap-out mechanism, and directly evicts KV caches based on the LRU policy when HBM is full.
To ensure a fair comparison, we extended vLLM to use main memory for storing history KV caches, implementing a swap-out mechanism based on the LRU policy when HBM is insufficient and pre-fetching them back when HBM memory becomes available.
 
    \item \textbf{S-LoRA:}
S-LoRA supports batched Multi-LoRA inference and uses a unified memory pool for LoRAs and KV caches.
However, S-LoRA does not reuse history KV caches and discards them after queries are completed.
For LoRAs, S-LoRA adopts an on-demand swapping mechanism, swapping in required weights during inference and swapping them out afterward to free up HBM memory for KV caches.
\end{enumerate}


\textbf{Metrics.} Following prior work~\cite{xx}, LLM inference in two stages: prefill and decode, so the performance of an LLM system is primarily determined by two metrics: \textit{Time to First Token (TTFT) and Time Per Output Token (TPOT)}. TTFT is the response time for generating the first token, and TPOT is the average time to generate each token after the first one. Additionally, we define \textit{peak throughput} as the maximum number of queries each system can complete per second without severe backlog, meaning when the average TTFT remains below 500ms. 
% We record the number of queries each system can complete per second on average at peak rate as \textit{peak throughput}.

\subsection{Application Scenarios}
We constructed three commonly seen large model inference scenarios based on real-world loads: chatbots, multi-language translation, and personal agents. For each scenario, we construct the experiment with various LoRA numbers and sending rates.

\textbf{Chatbots.}
Chatbots are the most common and important application of LLM inference. In each round chatbots use all the user's previous history to generate new output. Online services typically allow users to choose specific scenarios for conversation, such as mathematical calculations~\cite{}, business analysis~\cite{}, etc, and these multi-scenario services always leverage Multi-LoRA inference to increase inference efficiency and user experience.

We constructed queries based on the LMSYS-33k dataset~\cite{}. LMSYS-33k is an open-source dataset by the LMSYS organization containing 33,000 dialogues with real human preferences. Each sample includes the model name which query uses, the complete dialogue text, timestamps, and other information.
% The dataset contains 20 LLMs on Chatbot Arena, including powerful models like GPT-4 and Claude-v1.
According to model name, we constructed the target LoRA of each query and maintained the original model distribution. Also, We proportionally scaled the LMSYS-33k dataset on the time axis to achieve different average query sending rates while maintaining the original sending rate type, similar to previous work~\cite{}.

% We set the duration of each test round $T\_round$ to 600s. Suppose the desired average sending rate for the test round is one query per second. In that case, we select the first 600 queries from the LMSYS-33k dataset and calculate the difference in timestamps between the first and the 600th query $T\_diff\_total$, and the difference in timestamps between the $i$th and the $i+1$th query $T\_diff_{i+1}$. The time scaling factor $Scale\_Rate$ is:
% \begin{equation}
% \label{eq:time_scale_rate}
% Scale\_Rate=\frac{T\_round}{T\_diff\_total}
% \end{equation}
% During the experiment, we send the first 600 queries sequentially, where the interval $Interval_i$ between the $i$th and the $i+1$th query is:
% \begin{equation}
% \label{eq:interval}
% Interval_i = T\_diff_{i+1} \times Scale\_Rate
% \end{equation}
\textbf{Translations.} LLMs are increasingly used in translation tasks. Although open-source large models are usually based on corpora from various language, due to the unbalanced distribution, they do not perform well at any translation task. Researchers generally fine-tune the model to improve performance in certain languages, and the multi-language translation service providers can use Multi-LoRAs technique to dynamically select and use the target model to enhance translation results.

We construct query based on OPUS-100 dataset~\cite{xx}, which is a multi-language corpus covering 100 languages. It contains approximately 55 million sentence pairs. 
% The OPUS collection includes various types of corpora, such as movie subtitles, GNOME documents, and the Bible.
When inferencing, each language translation pair corresponds to a specific LoRA model. Because OPUS-100 dataset does not include query timestamps, we sample the arrival pattern of queries based on the production traces MAFT, Microsoft Azure function trace ~\cite{xx}, similarly as previous work~\cite{xx}. We sort the functions by call frequency, select the top $n$ queries, and map them to the $n$ LoRA models to maintain the queries' distribution.

% To improve translation effectiveness, current work typically constructs specific templates to specify the target language, style, and other information for translation. We referred to the Expert Language Translator~\cite{expert-language-translator} for construction, with specific instructions as shown in Table~\ref{tab:translation_template}.

\textbf{Personal agents.}
Personal agents aim to provide customized and intelligent support such as checking the weather, booking restaurants, and planning trips. Nowadays, LLMs have been widely applied in personal agents such as mobile smart assistants and home assistants. Also, Multi-LoRA is widely used for this typical multi-task serving.

We utilize Taskmaster~\cite{xx} to construct queries. Released by Google, Taskmaster is a conversational dataset designed to train and evaluate task-oriented dialogue systems, covering various real-world scenarios. Taskmaster features multi-turn dialogues with complex context management and information exchange, reflecting how people interact with assistants or others to complete tasks in real life. We use the same sample methods based on MAFT the same as multi-language translations.
\subsection{Latency and Peak Throughput}
% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/evaluation/big_ttft.pdf}
%     \includegraphics[width=1\linewidth]{Figures/evaluation/big_tpot.pdf}
%     % \includegraphics[width=1\linewidth]{Figures/evaluation/big_TP.pdf}
%     \caption{TTFT, TPOT of ELoRA and baseline in various scenarios. X-label means model size and LoRA number of experiment group respectively \SJC{Need modify throughput} \hang{need merge TTFT and TPOT and TP of each scenario later}}
%     \label{fig:eval_big}
% %    \vspace{-3mm}
% \end{figure*}

\begin{figure*}[htbp]
    \centering
    % 第一行
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_chatbot_ttft.pdf}
        % \caption{Image 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_translation_ttft.pdf}
        % \caption{Image 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_assis_ttft.pdf}
        % \caption{Image 3}
    \end{subfigure}

    % \vspace{-3pt}

    % 第二行
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_chatbot_tpot.pdf}
        % \caption{Image 4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_translation_tpot.pdf}
        % \caption{Image 5}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_assis_tpot.pdf}
        % \caption{Image 6}
    \end{subfigure}

    % \vspace{-3pt}

    % 第三行
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_chatbot_TP.pdf}
        \caption{Chatbot}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_translation_TP.pdf}
        \caption{Translation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\textwidth]{Figures/evaluation/big_assis_TP.pdf}
        \caption{Assistant}
    \end{subfigure}
    \caption{TTFT, TPOT of ELoRA and baseline in various scenarios. X-label means model size and LoRA number of experiment group respectively \hang{change y-licks}}
\end{figure*}


% \begin{figure}
%     \centering
%     \includegraphics[width=.8\linewidth]{Figures/evaluation/big_TP_chatbot.pdf}
%     \includegraphics[width=.8\linewidth]{Figures/evaluation/big_TP_translation.pdf}
%     \includegraphics[width=.8\linewidth]{Figures/evaluation/big_TP_assis.pdf}
%     \caption{Normalized peak throughput of \sysname{} and baselines in different experiment groups, each throughput is normalized according to vLLM so the red line is vLLM.}
%     \label{fig:eval_hbm} 
%     \vspace{-3mm}
% \end{figure}

We compared ELoRA with two baselines in three different scenarios. For each scenario, We construct an experiment group including various model size and LoRA numbers. For each experiment group we change query rate from 0 to peak throughput. The average results of each experiment group are shown in Figures~\ref{fig:eval_big}.

In all groups, our system achieved lower TTFT and TPOT compared to the baselines. For the chatbot scenario, our system reduced TTFT by an average of 58.0\% and TPOT by 28.3\% compared to vLLM, and reduced TTFT by 26.6\% and TPOT by 23.5\% compared to S-LoRA. For the multi-language translation scenario, our system reduced TTFT by an average of 68.9\% and TPOT by 51.7\% compared to vLLM, and reduced TTFT by 42.6\% and TPOT by 30.7\% compared to S-LoRA. For the personalized assistant scenario, our system reduced TTFT by an average of 55.3\% and TPOT by 21.8\% compared to vLLM, and reduced TTFT by 81.0\% and TPOT by 47.5\% compared to S-LoRA.

Additionally, we evaluated the throughput of each system at peak sending rates. In the chatbot scenario, our system achieved a 34.1\% throughput improvement compared to vLLM and a 19.2\% improvement compared to S-LoRA. In the multi-language translation scenario, our system achieved a 147.7\% throughput improvement compared to vLLM and a 46.4\% improvement compared to S-LoRA. In the personalized assistant scenario, our system achieved a 40.1\% throughput improvement compared to vLLM and a 107.9\% improvement compared to S-LoRA.

\subsection{Breakdown of the Query Execution Time}

\subsection{HBM Utilization and Hit Rate}
\textit{Cache hit rate comparison.
Cold start time of queries for different systems.
Invalid memory blocks statistics.
Therefore, ELoRA can better reduce xxx.}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_gpu_chatbot.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_gpu_translation.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_gpu_assis.pdf}
    \caption{The average HBM usage of \sysname{} and baseline in different experiment group.}
    \label{fig:eval_hbm} 
    \vspace{-3mm}
\end{figure}

\textbf{HBM utilization.} We analyze the utilization of HBM resources across different experimental groups, as shown in Figure\ref{fig:eval_hbm}. Compared to vLLM and S-LoRA, \sysname{} achieve significantly higher HBM resource utilization. For S-LoRA, due to the inability to leverage history KV caches, the HBM utilization remains low throughout the inference process, leaving a large portion of HBM idle. For vLLM, although it can utilize history KV caches, it cannot dynamically scale the LoRA memory pool and KV memory pool. As a result, under dynamic experiments where the sending rate and distribution continuously change, unused HBM space inevitably occurs. In contrast, \sysname{} can dynamically adjust the allocation ratio between LoRAs and KV caches and promptly preload KV caches and LoRAs into idle HBM. 
% Consequently, ELoRA achieves higher HBM utilization across all experimental groups. 
We also shows HBM usage during dynamic load in section\ref{sec:breakdown}.

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_hit_chatbot.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_hit_translation.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/big_hit_assis.pdf}
    \caption{The hitted rate of \sysname{} and baseline in different experiment group.}
    \label{fig:eval_hitted} 
    \vspace{-3mm}
\end{figure}

\textbf{Hitted rate and breakdown.} We analyze the cache hit rate of various experimental groups, as shown in Figure~\ref{fig:eval_hitted}. We observe that, due to the more efficient memory block swapping strategy adopted by LogicLoRA, it is possible to prefetch the optimal KV cache and LoRAs into HBM more effectively. Consequently, when a query arrives, the cache hit rate is higher, which reduces the overhead of swapping, as illustrated in Figure~\ref{xx} \hang{(How to show?)}. Compared to vLLM and S-LoRA, our approach achieves lower cold-start latency for LoRAs and KV cache.

\begin{figure}[htbp]
    \centering

    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/evaluation/dynamic_HBM_ours-best.pdf}
        \caption{\sysname{}}
        \label{fig:dynamic_hbm_ours_best}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/evaluation/dynamic_HBM_vllm.pdf}
        \caption{vLLM}
        \label{fig:dynamic_hbm_vllm}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/evaluation/dynamic_HBM_slora.pdf}
        \caption{S-LoRA}
        \label{fig:dynamic_hbm_slora}
    \end{subfigure}
    
    \caption{The breakdown of HBM allocation of \sysname{} and baseline in different experiment group. \hang{Need modify to explain on figure} \SJC{three systems in a figure.}}
    \label{fig:dynamic_hbm} 
    \vspace{-3mm}
\end{figure}

\subsection{Breakdown of the HBM Allocation}
\label{sec:breakdown}
Examples to compare HBM memory allocations for KV and LoRAs of different systems (HBM using rate for KV/LoRA with time.)

Figure~\ref{fig:dynamic_hbm} illustrates the HBM management status of ~\sysname{} and baselines during a serving process(chatbot, LoRA number is 100, average send rate is 1.6, model is Llama-13B). 

For ELoRA, during the first 400 seconds(a) with low HBM pressure, the performance-driven cache swapper proactively prefetches all LoRAs into HBM to eliminate the cold-start overhead of LoRAs. In contrast, both vLLM and S-LoRA ignore this process, leading a higher TTFT. S-LoRA also destroys all history KV cache and makes TTFT worse.
After 400 seconds(b), as the query rate increases, ELoRA begins to swap-out LoRAs and history KV cache blocks to free up more space for current inference, and the running KV cache is close to 100\%, thus avoiding insufficient KV caches. However, for vLLM, the static memory allocation strategy results in the KV cache memory pool being filled to its maximum capacity (close to 80\%). This prevents further allocation of space for running KV cache, leading to queuing and the rapid growth of TTFT.
During later inference stages(c), ELoRA remains a significant number of hot LoRAs and portions of history KV cache in HBM to reduce cold-start latency when queries arrive. However, due to the lack of previous KV pools, vLLM retains less history KV on HBM.

% For vLLM, although it considers the retention of history KV cache(a), after 400 seconds(b), the static memory allocation strategy results in the KV cache memory pool being filled to its maximum capacity (close to 80\%). This prevents further allocation of space for running KV cache, leading to queuing and the rapid growth of TTFT. In contrast, ELoRA, with its unified management mechanism for LoRAs and KV cache, can evict LoRAs to allocate more space for current inference, thus avoiding insufficient KV caches. 

% For S-LoRA, since it neglects the retention of history KV cache, HBM memory is only used to store running LoRAs and KV cache. As a result, there is a large amount of unused HBM memory throughout the entire process. Additionally, compared to ELoRA, S-LoRA lacks a prefetching mechanism for LoRAs and does not retain hotspot LoRAs, further leading to idle HBM memory space and higher cold-start latency. 

Therefore, compared to vLLM and S-LoRA, ELoRA achieves more efficient memory swapping for LoRAs and KV cache, resulting in higher memory utilization and better end-to-end performance. \hang{checked above}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_chatbot_ttft.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_translation_ttft.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_assis_ttft.pdf}
    \caption{TTFT of \sysname{} and ablation study results in different experiment group.}
    \label{fig:abl_ttft} 
    \vspace{-3mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_chatbot_tpot.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_translation_tpot.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/abl_assis_tpot.pdf}
    \caption{TPOT of \sysname{} and ablation study results in different experiment group.}
    \label{fig:abl_tpot} 
    \vspace{-3mm}
\end{figure}

\subsection{Efficiency of the Logic-aware Cache Manager}
Show results of ELoRA without tree-based memory structure.

To demonstrate the efficiency of the Logic-aware Cache Manager, we compared ELoRA with the results after removing this structure. We constructed ELoRA-WOT, which still uses a unified memory pool to manage LoRAs and KV cache, but does not perceive or maintain the relationship between LoRAs and KV cache. 
% Therefore, although ELoRA-WOT actively swaps LoRAs and KV cache based on preset thresholds, it does not follow the logical order between LoRAs and KV cache during swapping. 
Instead, it scores LoRAs and KV cache separately using the cost model and proportionally selects the highest benefit LoRAs and KV cache for swapping. We tested ELoRA-WOT in previously mentioned task scenarios and compared it with the complete ELoRA. The results are shown in Figure~\ref{fig:abl_ttft}. 
Experiments show that for chatbots, multi-language and personal assistants, ELoRA-WOT exhibited 19.6\%, 28.1\%, 33.8\% average increase in TTFT respectively. We also find the ELoRA-WOT exhibited 14.0\%, 20.7\%, 19.4\% average increase in TPOT, respectively, shown in Figure~\ref{fig:abl_tpot}.

% average increase in TTFT and a 14.0\% average increase in TPOT compared to ELoRA. In the multilingual translation experimental group, ELoRA-WOT exhibited a 28.1\% average increase in TTFT and a 20.7\% average increase in TPOT compared to ELoRA. In the personalized translation experimental group, ELoRA-WOT exhibited a 33.8\% average increase in TTFT and a 19.4\% average increase in TPOT compared to ELoRA.


% \subsection{Efficiency of the Least LoRA Number Guarantee}
% Show results of ELoRA without the LoRA number satisfied.

\SJC{Devide Section-6.6 into two subsections, without lora, without cache swapper}

\subsection{Efficiency of the Performance-driven Cache Swapper}
Show results of ELoRA without the cost model (LRU).

To demonstrate the efficiency of the performance-driven cache swapper, we replace it with a simply LRU module and get ELoRA-WOC. Specifically, when swapping in, ELoRA-WOC prioritizes the node that was used the least recently, and when swapping out, it prioritizes the node that was used the most recently. We tested ELoRA-WOC in the previously mentioned task scenarios and compared it with the complete ELoRA. The results are shown in Figures~\ref{fig:abl_ttft}. 
Experiments show that for chatbots, multi-language and personal assistants, ELoRA-WOC exhibited 12.9\%, 16.5\%, 14.7\% average increase in TTFT respectively. We also find the ELoRA-WOC exhibited 9.7\%, 19.6\%, 11.2\% average increase in TPOT, respectively, shown in ~\ref{fig:abl_tpot}.

% Experiments show that in the chatbot experimental group, ELoRA-WOC exhibited a 12.9\% average increase in TTFT and a 9.7\% average increase in TPOT compared to ELoRA. In the multilingual translation experimental group, ELoRA-WOC exhibited a 16.5\% average increase in TTFT and a 19.6\% average increase in TPOT compared to ELoRA. In the personalized translation experimental group, ELoRA-WOC exhibited a 14.7\% average increase in TTFT and an 11.2\% average increase in TPOT compared to ELoRA.


\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{Figures/evaluation/extend_test_TTFT.pdf}
    \includegraphics[width=.8\linewidth]{Figures/evaluation/extend_test_TPOT.pdf}
    \caption{TTFT and TPOT of \sysname{} and baseline with extended LoRA number and distributions.}
    \label{fig:extend} 
    \vspace{-3mm}
\end{figure}

\subsection{Impact of LoRA Number and Distribution}
Change LoRA number to 1000+ and different distribution, to explain we have best performance all the time.

To demonstrate the generalizability of the ELoRA system, we further expanded the number and distribution of LoRAs used in the experiments. Referring to the configurations of previous works\cite{xx,xx}, our experimental group includes 2000 types of LoRAs and extreme types of LoRA distributions. We set the LoRA distributions as follows: \textbf{1. Uniform,} where the proportion of each LoRA weight is equal. \textbf{2. Distinct,} where each query uses a distinct LoRA. \textbf{3. Skewed-x,} where the proportion of queries selecting each LoRA weight varies. We constructed queries based on a Gaussian distribution and set different standard deviations \textbf{x}. The results are shown in figure~\ref{fig:extend}. Our system still achieves significant end-to-end performance improvements compared to the baseline these expanded experimental group, demonstrating the generalizability of our system.


% \subsection{Performance Results on GPUs}
% Show the results on GPUs.

\subsection{Overhead of ELoRA}

We measured and evaluated the overhead introduced by the Logic-LoRA system. Specifically, Logic-LoRA introduces three types of overhead: the overhead of logic tree matching, multiplexing, and insertion updates; the overhead of monitoring memory usage; and the balancing overhead of the memory block scheduler.

For the logic tree, we employ an efficient dictionary prefix tree structure for rapid matching. We found that even when HBM resources are fully utilized and the nodes in the tree reach their maximum, the average overhead for indexing and searching in the logic tree is less than 0.5 ms. Compared to the entire inference process, which can take seconds or even tens of seconds, this overhead is negligible. The insertion and update of the logic tree are merely updates to the dictionary prefix tree structure and do not involve actual memory operations, resulting in very low overhead, with an average of less than 1 ms.

For monitoring memory usage, we utilize an independent thread, which introduces no additional overhead. Similarly, the balancing of the memory block scheduler is done through an independent thread that monitors and obtains memory block exchange plans. We perform asynchronous transmission of memory blocks, overlapping the memory block transfer process with the inference process. Thus, the balancing process does not affect the current inference process and introduces almost no additional overhead.


==> Sections/implementation.tex <==
\section{Implementation of \sysname{}}
In this section, we describe how \sysname{} establishes unified the HBM and main memory pool for LoRAs and KVs, as well as implementing the usage dependency tree.

\subsection{Unified HBM Pool for LoRAs and KVs}
\SJC{State compared to vLLM, how to implement the unified memory pool.}
To achieve a unified memory pool for HBM and main memory, we have extended the BlockManager of vLLM. During the initialization phase, both HBM and main memory are partitioned into memory blocks of the same size. We perform block-wise partitioning of LoRA weights along the Rank dimension. Since the other dimensions of LoRA align with those of the KV cache, this approach ensures full alignment with the KV cache and avoids fragmentation. Based on the partitioning results, Logic-LoRA unified allocates memory to the KV caches and LoRsA at the granularity of blocks. When LoRA or KV cache entries are invalidated, Logic-LoRA recycles the corresponding memory blocks to the memory pool for future allocation.

\subsection{Usage Dependency Tree}
\SJC{Add implementations on how to implement the dependency tree.}

==> Sections/intro-V2.tex <==
\section{Introduction}

%\quan{Directly introduce the background of Multi-LoRA, KV-Cache in the first paragraph.}
Large Language Models (LLMs) are now widely used to understand and generate human-like text~\cite{mann2020language,chowdhery2023palm}. 
While it is cost inefficient to train LLMs for different tasks,  parameter-efficient fine-tuning~\cite{xx,xx} that frozes the large scale base model and 
fine tunes multiple Low-Rank Adapters (LoRAs) for different tasks are widely used currently~\cite{xx,xx}. 
For instance, in applications like chatbot~\cite{ChatGPT,Bard}, personal agents~\cite{xx,xx}, and multi-language translation~\cite{xx,zhang2016google},
multiple LoRAs can be tuned for different user languages and application scenarios. 
For these LLMs, Key-Value (KV) caches that store input context are often used to maintain coherence and speed up responses during extended interactions by avoiding repetitive computations~\cite{xx,xx}.
Researchers also proposed to reuse history KVs for queries with the same prefix~\cite{zheng2023efficiently,gim2024prompt,yao2024cacheblend,yu2023stateful}, further boosting performance in iterative tasks.
To enable quick access to the base model, the LoRA adapters, and the KVs, are often cached in the high bandwidth memory(HBM) of accelerators (e.g., global memory of Nvidia GPUs
or global memory of various AI accelerators~\cite{a,b,c}).

\begin{comment}
Large Language Models (LLMs) are advanced AI systems designed to understand and generate human-like text~\cite{mann2020language,chowdhery2023palm}.
A key feature that improves the efficiency is the use of Key-Value (KV) caches, which store input context to maintain coherence and speed up responses during extended interactions by avoiding repetitive computations~\cite{xx,xx}.
History KVs can also be reused for queries with the same prefix~\cite{zheng2023efficiently,gim2024prompt,yao2024cacheblend,yu2023stateful}, further boosting performance in iterative tasks.
LLMs also excel at adapting to specific tasks using parameter-efficient fine-tuning~\cite{xx,xx}, in which Multi-LoRA is a popular method that applies separate Low-Rank Adapters (LoRAs) to different queries while sharing the same base model~\cite{xx,xx}. This approach allows for flexible and efficient adaptation without extensive retraining, supporting applications like chatbot~\cite{ChatGPT,Bard}, personal agents~\cite{xx,xx}, and multi-language translation~\cite{xx,zhang2016google}.
\end{comment}

Many works have investigated to cache the base model, the KVs~\cite{xx,xx,xx} or ``hot'' LoRA adapters (LoRAs in short)~\cite{xx,xx,xx}, while the HBM size is limited.
While caching both KVs and LoRAs can improve inference performance, vLLM~\cite{xx} and SGLang~\cite{xx} proposed to cache both LoRAs and KVs.
\autoref{fig:intro} shows an example of caching base model, LoRAs, and KVs. 
Specifically, LoRAs have seperate KV caches (e.g., LoRA-1 and LoRA-2 have independent KV caches), the HBM space is statically partitioned and assigned for caching LoRAs and KVs.
When a user query is received, the serving system checks whether the required LoRA and KVs are already in the HBM or not. 
If the required LoRAs and/or KVs are not cached, they are swapped in from the main memory. If the cache space for the LoRAs/KVs is full, some of them 
are swapped out with various caching policies.

%While caching both KVs and LoRAs can improves inference performance but increases contention under limited HBM space, the above works have not explored solutions for caching them together.
\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/intro-new-4.pdf}
    \caption{An example caching state to show the \textbf{\textit{Usage dependencies}} between LoRAs and KV caches.}
    \label{fig:intro}
    \vspace{-3mm}
\end{figure}

\begin{comment}
\quan{Introduce the existing caching mechanisms for Multi-LoRA and KV-Cache due to the limited accelerator HBM, in terms of optimizing TTFT and TPOT.}
Many works have widely investigated to cache the KVs~\cite{xx,xx,xx} or ``hot'' LoRAs~\cite{xx,xx,xx} in the High Bandwidth Memory (HBM) on accelerators like GPUs and NPUs, to improve the query inference performance in terms of optimizing the Time-To-First-Token (TTFT) and Time-Per-Output-Token (TPOT).
% Facing the Multi-LoRA inference scenario, some other works also pre-cached the ``hot'' LoRAs in the HBM to improve the inference performance~\cite{xx,xx,xx}.
Moreover, they adopted the Least Recently Used (LRU) for pre swapping-in/out LoRAs or KV caches.
While caching both KVs and LoRAs can improves inference performance but increases contention under limited HBM space, the above works have not explored solutions for caching them together.
\end{comment}

%叫做pre-cache xxx？
%\quan{The inefficiencies of current caching mechanism. It is better to also have some data support. Like, the increase of TTFT, etc.}

\begin{comment}
To address the Multi-LoRA inference scenario, some of current LLM inference frameworks (like vLLM~\cite{xx} and SGLang~\cite{xx}) have integrated the functionlity to manage the caching for both KVs and LoRAs in the HBM, and they partitioned fixed HBM space for KV cache and LoRAs separately.
% Some of current LLM inference frameworks (like vLLM~\cite{xx} and SGLang~\cite{xx}) have integrated the LoRA caching in HBM, and they partitioned fixed HBM space for KV cache and LoRAs separately.
However, a static partition only performs well in a fixed distribution of queries to access different LoRAs. It will lead to HBM underutilized with many cold-start LoRAs or KV caches at other cases.
Our investigations show that vLLM with default HBM partition increases the TTFT by up to \textcolor{red}{xx.x\%} compared to the brute-force achieved oracle HBM partition.
Even if unified managing both the history KV caches and LoRAs in the HBM, the inference performance is still not efficient and the reasons are from two aspects.
\end{comment}
% Moreover, some other works (like S-LoRA~\cite{xx}) unified managed LoRAs and running KV caches in HBM at the block level. They did not consider the history KV caches in the HBM, increasing the recomputation overhead in multi-turn interactions.

If queries use different LoRAs following stable distributions, the above solution performs well because the optimal HBM space partition can be identified in a ``brutal-force'' way.
However, production traces~\cite{xx,xx,xx} show that the distributions are dynamic. 
In such scenario, we observe that static HBM space partition and independent cache management suffers from low efficiencies in both intra-LoRA aspect 
and inter-LoRA aspect. 

In the intra-LoRA aspect, it is possible that a query's KVs are cached while the required LoRA is swapped out.
For a single LoRA's query, as shown in \autoref{fig:intro}, when a query ``Query-1'' that relies on LoRA-1 arrives, it can run only if both LoRA-1 and the prefixed KV1-1 and KV1-2 are already in the HBM.
However, LoRA-1 are swapped out earlier due to the limited HBM space.
In this case, the cached KVs are actually ``invalid'', because the query cannot run without the required LoRA.
In the inter-LoRA aspect, the ``invalid'' KVs of a LoRA may prevent useful KVs of other LoRAs from being cached. 
For instance, KV2-2 are not cached in the HBM, though KV1-1 isk actually invalid. 
In this case, the query that relies on LoRA-2 cannot run as well.
Our evaluations show that the vLLM can have up to \textcolor{red}{50.x\%} invalid KV caches.

\begin{comment}
The Query-1 needs to first match the LoRA-1 and then match the subsequent KV1-1 in the HBM, representing the logic dependencies between LoRAs and KV caches.
However, under this caching state, Query-1 has to wait for the LoRA-1 to be swapped-in although its required KV1-1 exist.
During LoRA-1's cold-start, the ``invalid'' KV1-1 occupies HBM without being utilized, preventing other queries' required KVs or LoRAs from loading, e.g., the KV2-2, thereby harming the HBM utilization and inference performance.
Our evaluations show that the vLLM can have up to \textcolor{red}{50.x\%} invalid KV caches.
\end{comment}

%However, a static partition only performs well in a fixed distribution of queries to access different LoRAs. It will lead to HBM underutilized with many cold-start LoRAs or KV caches at other cases.
%Our investigations show that vLLM with default HBM partition increases the TTFT by up to \textcolor{red}{xx.x\%} compared to the brute-force achieved oracle HBM partition.
%Even if unified managing both the history KV caches and LoRAs in the HBM, the inference performance is still not efficient and the reasons are from two aspects.



%我们改成matching dependency?
%\quan{The root cause is neglecting the usage dependency, order dependency? logic dependency is not a good phrase. }

The above inefficiencies originate from neglecting the usage dependencies of LoRAs and KVs, and the load variation of LoRAs.
This work has two key insights. First, an mechanism is required to integrate the usage dependency for each LoRA adapter and its KVs into the caching strategy.
By such means, we can keep valid KVs in HBM as much as possible to improve the HBM efficiency.
Second, reserving sufficient HBM space for LoRAs help in improving peak throughput, while it may hurt the Time-To-First-Token (TTFT) and Time-Of-Per-Token(TOPF) of each single query.
A scheme is required to manage the HBM space used by different LoRAs and their KVs.
It is challenging to achieve such design to balance the usage of LoRAs and KVs, because XXXXXXXX.


\begin{comment}
Firstly, these works ignored the \textbf{logic dependencies} between LoRAs and KV caches. 
Figure~\ref{fig:intro} shows an example caching state under the Multi-LoRA scenario, abstracted from using the vLLM~\cite{vLLM2023}.
As shown, LoRA-1 and LoRA-2 have their independent KV caches although KV1-1 and KV2-1 have the same token due to the calculation with different LoRA branches.
The Query-1 needs to first match the LoRA-1 and then match the subsequent KV1-1 in the HBM, representing the logic dependencies between LoRAs and KV caches.
However, under this caching state, Query-1 has to wait for the LoRA-1 to be swapped-in although its required KV1-1 exist.
During LoRA-1's cold-start, the ``invalid'' KV1-1 occupies HBM without being utilized, preventing other queries' required KVs or LoRAs from loading, e.g., the KV2-2, thereby harming the HBM utilization and inference performance.
Our evaluations show that the vLLM can have up to \textcolor{red}{50.x\%} invalid KV caches.
%这里说出来我们发现了LoRA caching的作用，
Secondly, we observe that sufficient pre-cached LoRAs can support higher peak serving throughput, and other metrics that benefit to inference performance \textcolor{red}{(like xxx and xxx)} need to be considered for reducing TTFT and TPOT.
However, current caching systems utilized the LRU strategy which neglects our above observations.
\end{comment}

%\quan{The challenges are: 1) how to integrate the dependency into caching; 2) Lora adapter or KV-cache, which is more important for TTFT or TPOT? 3) swap in and out. Also mention why they are challenges.}

\begin{comment}
To address the above problems, two challenges exist for efficient caching of KVs and LoRAs under the Multi-LoRA serving scenario.
Firstly, an appropriate caching scheme needs to be integrated for maintaining the logic dependencies between LoRAs and KVs in the HBM. By such means, we can keep valid KV caches in HBM as much as possible to improve the HBM utilization efficiency, and thus the TTFT and TPOT of query inference can be optimized.
%体现出来我们说的两阶段,先保证吞吐,再优化TTFT和TPOT,
Secondly, on top of the caching scheme, sufficient HBM space for LoRAs needs to be reserved to enhance the peak throughput. Moreover, a cost model with comprehensive metrics to optimize the TTFT and TOPT is required for deciding the KV and LoRA swap-in/out, to reduce cold-start time during query inference.
\end{comment}


%\quan{We therefore propose \sysname{}, xxxxxx. , XXX organizes the lora adapter and kv cache. }

% \SJC{Why our cost model is not constust based on TPOT?}

Based on the two insights, we therefore propose \textbf{\sysname{}}, a Multi-LoRA inference caching system that optimizing the caching of LoRAs and KVs considering usage dependency.
\sysname{} aims to maximize the peak serving throughput, while reducing the TTFT and TOPT of multi-LoRA applications.
It consists of a \textit{logic-aware cache manager} and a \textit{two-stage cache swapper}.
The cache manager maintains the logic dependencies between KV caches and LoRAs based on a well-designed tree-based scheme, where nodes are KV caches or LoRAs and edges are their dependencies. 
To maintain the logic dependencies during the inference, LoRAs or KV caches are inserted or eliminated from leaves to keep the tree connected.
After each monitor interval, the cache swapper first loads the minimum required number of LoRAs into HBM to support higher peak throughput.
Then, it decides the swapping-in/out LoRAs or KV caches based on a cost model when the HBM is idle and busy, respectively. 
This model define the cost as the expected decrease/increase in the TTFT for future queries.
\quan{How the cost model is build. What are the inputs/outputs of the cost model.}

\begin{comment}
We therefore propose \textbf{\sysname{}}, a Multi-LoRA inference caching system that organizes the LoRAs and KV caches in the HBM.
It consists of a \textit{logic-aware cache manager} and a \textit{two-stage cache swapper}.
The cache manager maintains the logic dependencies between KV caches and LoRAs based on a well-designed tree-based scheme, where nodes are KV caches or LoRAs and edges are their dependencies. 
To maintain the logic dependencies during the inference, LoRAs or KV caches are inserted or eliminated from leaves to keep the tree connected.
After each monitor interval, the cache swapper first loads the minimum required number of LoRAs into HBM to support higher peak throughput.
Then, it decides the swapping-in/out LoRAs or KV caches based on a cost model when the HBM is idle and busy, respectively. 
This model define the cost as the expected decrease/increase in the TTFT for future queries.
% This model considers the metrics of recent access time, frequency, and swap-in/swap-out overheads, and define the cost as the expected decrease/increase in the TTFT for future queries.
\end{comment}

\quan{The contributions.}

This paper makes three major contributions.
\begin{itemize}
    \item \textbf{Investigating the caching management of LoRAs and KVs for the Multi-LoRA inference.} The analysis motivates us to maintain the logic dependencies between LoRAs and KV caches during inference, and comprehensively considers the metrics related to inference performance for their swapping-in/out.
    % fully considers performance metrics for their swapping-in/out.
    \item \textbf{A cache manger to maintain the logic dependencies between LoRAs and KV caches.} The manager adopts a tree-based scheme to construct the dependencies, and inserts or eliminates nodes from the leaves. It maintains the logic dependencies to ensure the HBM fully utilized, and thus improve the query inference performance.
    \item \textbf{A cache swapper to swap-in/out appropriate LoRAs or KV caches.} 
    The swapper first reserves sufficient LoRAs in the HBM and then decides the swapped-in/out KVs or LoRAs based on a comprehensive cost model.
    It enhances the peak throughput and avoids the cold-start overhead during the inference.
\end{itemize}

%\quan{Our implementation and evaluation platform, results. }

We have implemented \sysname{} to top of the vLLM~\cite{xx} and evaluated it with Llama-7B/13B/34B models~\cite{touvron2023llama} on eight Atlas 300I NPUs~\cite{xx} with three typical scenarios (chatbot~\cite{luo2024arena,chiang2024chatbot}, multilingual translation~\cite{zhang2020improving}, and personal agents~\cite{xx}). Experimental results show that Logic-LoRA reduces the TTFT and TPOT by 63.4\% and 40.1\%, respectively, compared to state-of-the-art Multi-LoRA inference systems.


%问题汇总:
%TTFT主要提升，TPOT只是小方面，冗余计算少了 内存利用率高了 吞吐快了 ； 但是一般来说TTFT行了，TPOT自然也就好了
%做统一history kv和lora管理使我们的贡献？
%moti中用什么baseline
%是否要一直提Pre-caching
%为什么figure-3的oracle ratio旨在0.1-0.3之间？
%balance the usage of KV and LoRA没想好要如何写
%logic dependency的表达方式

%intra-LoRA: logic dependencies \ invalid KVs \ HBM under-utilization
%inter-LoRA: HBM allocation for LoRAs due to dynamic loads, swap-in/out which LoRA related KV caches

==> Sections/intro.tex <==
\section{Introduction}

\quan{Directly introduce the background of Multi-LoRA, KV-Cache in the first paragraph.}

\quan{Introduce the existing caching mechanisms for Multi-LoRA and KV-Cache due to the limited accelerator HBM, in terms of optimizing TTFT and TPOT.}

\quan{The inefficiencies of current caching mechanism. It is better to also have some data support. Like, the increase of TTFT, etc.}

\quan{The root cause is neglecting the usage dependency, order dependency? logic dependency is not a good phrase. }

\quan{The challenges are: 1) how to intergrate the dependency into caching; 2) Lora adapter or KV-cache, which is more important for TTFT or TPOT? 3) swap in and out. Also mention why they are challenges.}

\quan{We therefore propose \sysname{}, xxxxxx. , XXX organizes the lora adapter and kv cache. }

\quan{The contributions.}

\quan{Our implementation and evaluation platform, results. }

% \shi{Para.1: Background of LLM. A single application needs los of LLMs for different scenarios.}
The large language model (LLM) is widely deployed in user-facing applications to understand human language~\cite{mann2020language,chowdhery2023palm}, such as chatbot~\cite{ChatGPT,Bard}, virtual assistant~\cite{copilot,chen2021evaluating}, and machine translation~\cite{zhang2016google}. 
A LLM with a single functionality often needs multiple full-parameter training to adapt to different scenarios~\cite{xx,xx}, e.g., two respective training of Llama-3 is needed to chat to doctors and lawyers. Moreover, under the inference demand of users from various scenarios, deploying many LLMs with tens to hundreds of billion parameters consumes considerable High Bandwidth Memory (HBM) on GPUs or NPUs~\cite{xx,xx}.
With the limited HBM, the inference performance can be decreased due the resource competition~\cite{xx,xx}.

% \shi{Para.2: LoRA technique. Multi-tenant lora scenario, has benefits to deploying single LLM for each.}
The Low-Rank Adaptation (LoRA) is proposed under the above situation, which only needs to fine-tune a few low-rank matrices along with a base model to adapt to one inference scenario~\cite{hu2021lora,wang2024lora}.
%to adapt to various user inference scenarios
% with neglgible accuracy loss compared to full-parameter training
For serving queries from hundreds of scenarios, Multi-LoRAs are deployed with the same base model and the queries are batched to be processed~\cite{chen2024punica,sheng2024slora,wu2024dlora}.
The Multi-LoRA saves the HBM usage compared to deploy an individual LLM for each scenario, but it can also take up considerable HBM~\cite{xx,xx}, e.g., xxx LoRAs with xxxGB. 

% \shi{Para.3: KV cache and LoRA cache.}
Similar to Multi-LoRAs, running KV caches of the query being served also occupy the HBM space.
Moreover, queries with the same prefix can reuse the same history KV caches to reduce redundant computations~\cite{zheng2023efficiently,gim2024prompt,yao2024cacheblend,yu2023stateful}, e.g., multi-turn dialogue, and they can be cached in HBM to speedup the inference.
However, it is hard to satisfy the caching demand of LoRA and KV caches simultaneously due to limited HBM~\cite{xx,xx}.
Thus, some LoRAs or KVs need to be offloaded to host memory and loaded to HBM on-demand~\cite{xx,xx}, which brings the cold-start overhead.
This harms the Time-To-First-Token (TTFT) and Time-Per-Output-Token (TPOT)~\cite{xx,xx} for inference, and can be optimized by smartly pre-caching hot-pot LoRAs or KVs on HBM~\cite{gao2024attentionstore}.

% The pre-caching of KVs~\cite{aminabadi2022deepspeed,pope2023efficiently} and LoRAs~\cite{xx,xx} can improve the inference efficiency.
% With LLM's auto-regression, queries with the same prefix can reuse the same history KV caches to reduce redundant computations~\cite{zheng2023efficiently,gim2024prompt,yao2024cacheblend,yu2023stateful}, e.g., multi-turn dialogue.
% However, the HBM is limited relative to the KV demand, e.g., a query with \textcolor{red}{8000} tokens needs about \textcolor{red}{35.2GB} HBM, some KVs need to be offloaded to host memory~\cite{xx,xx}, bringing the cold-start of KVs. This can harm the inference performance like Time-To-First-Token (TTFT) and Time-Per-Output-Token (TPOT)~\cite{xx,xx}, and the cold-start overhead can be optimized by pre-caching hot-pot KVs~\cite{gao2024attentionstore}.
% Similar to KV caches, Multi-LoRAs also occupies considerable HBM space~\cite{sheng2024slora,li2024caraserve}, thus pre-caching appropriate LoRAs into HBM can benefit the inference performance~\cite{xx,xx}

\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/intro.pdf}
    \caption{An example pre-caching state to present the \textbf{\textit{logic dependencies}} between LoRAs and KV caches.\quan{Some legend should be added for helping in understand the figure. It is a little bit complex as the first figure. The mechanism should be introduced in the text.}}
    \label{fig:intro}
    \vspace{-3mm}
\end{figure}

% \shi{Para.4: new characteristics of unified KV and LoRA management.}
Figure~\ref{fig:intro} shows an example pre-caching state under Multi-LoRA scenario, abstracted from investigating current LLM inference systems~\cite{vLLM2023}.
We can observe that the same history KVs need to be separately cached for different LoRAs, e.g., LoRA-3 and LoRA-4 have the same ``Here comes the sun''.
A query's prefix matching also must be performed after the loading of its referred LoRA.
For the example Query-1, it fails to match its required LoRA-1 in HBM, and has to wait for LoRA-1's cold swapped-in, although its required KVs already cached in the HBM (\ding{172}).
After the cold-start time of LoRA-1, this query matches three KV caches that refer to LoRA-1, and then the KV cache ``no'' is swapped-into the HBM (\ding{173}). 
At last, this query calculates the next token (\ding{174}).
Above workflow presents the \textbf{\textit{logic dependencies}} between LoRAs and KVs.

% shi{Para.6: Current works.}
Some LLM inference systems (e.g., vLLM~\cite{vLLM2023}) partitioned the HBM for KV cache and LoRAs separately.
However, a static partition only performs well in a fixed distribution of queries to access different LoRAs. It will lead to HBM underutilized with many cold-start LoRAs or KV caches at other cases.
Some other works~\cite{chen2024punica,sheng2024slora,xxx} unified managed LoRAs and KV caches in HBM at the block level, and adopted the Least Recently Used (LRU) for pre swapping-in/out LoRAs and KV caches.
They still have poor inference inefficiency with TTFT and TPOT, and the reasons are from two aspects.

% \shi{Para.5: As for the first reason, fixed HBM allocation has poor adaptability in various dynamic scnearios, and a fixed static allocation is often only suitalbe for one type of lora distribution (number/distribution/load).}
% As for the first reason, the static HBM partition fails to adapt to dynamic changing of the distribution of queries for different LoRAs.
% The static management cannot dynamically adjust the memory allocation for LoRAs or KV caches, and 
% A static partition only performs well under a specific distribution, and thus it will lead to HBM underutilized with more cold-start LoRAs or KV caches at other cases, resulting in low inference efficiency.

% \shi{Para.6: As for the second reason, even if unified management, lacking the awareness of logical relationships leads to ``invalid blocks'' and ``low cache hist rates'' in HBM. Explain what is ``invalid blocks'' in Figure1,a dn provide data with a low cache hit rate.}
As for the first reason, these works ignorde the logic dependencies between LoRAs and KV caches. This leads to unreasonable pre swapping-in/out with many ``invalid'' KV caches in HBM.
% which decreases the KV cache reuse during the inference. 
As shown in Figure~\ref{fig:intro}, Query-1 has to wait for the LoRA-1 to be swapped-in although its required KV caches exist. During LoRA-1's cold-start, these ``invalid'' KV caches occupy HBM space without being utilized, preventing other queries' required KVs or LoRAs from loading, thereby reducing the HBM utilization efficiency and inference performance.
Our evaluations show that the Multi-LoRA inference system VLLM can have up to \textcolor{red}{50.x\%} invalid KV caches.
% making the average cache block cold start time increase by xxxms.

% \shi{Para.7: As for the third reason, appropriate pre-swap-in/out strategy is necessary. A simpel LRU based strategy does not work in multi-tenant lora, because we find that we should first satisfy the demand for the lora number to avoid cold start. Moreover, we need to consider more factors like frequency and time overhead to swap-in/out blocks. Some data examples to show LRU is not good, some blocks' frequency is high but is swapped-out.}
As for the second reason, the LRU strategy usually pre swaps-in/out inappropriate LoRA and KV caches.
First, the LRU may lead remaining HBM space to not satisfy the minimum demand of LoRAs. Since the inference can only be proceed once required LoRAs are loaded into HBM, it decreases the supported peak throughput. 
Second, the LRU neglects other significant metrics that are sure to benefit for inference performance (frequency, swap-in/out and re-computation overheads), thus inappropriate swapping-in/out is performed.
%这些performance metrics和冷启动都有关系

% \shi{Para.8: An intuitive method is to unified manage the KV and Lora in HBM, perceive the logical relationship between KV and Lora, and carefully make decisions to swap-in/out cache blocks. However, it is necessary to utilize an appropriate cache management structure to maintain the relationship between KV and loras, enabling logical guidance for swap-in/out cache blocks under dynamic scenarios. Moreover, a cost model needs to be defined to comprehensively evaluate the priority of scheduling cache blocks swap-in/out HUB based on various metrics.}
A feasible solution is to explore an appropriate structure to construct and maintain the logic dependencies between LoRAs and KV caches. By such means, we can keep valid KV caches in HBM as much as possible, which can enhance the HBM utilization efficiency.
Based on this structure, a cost model with full performance metrics is also needed to decide appropriate swapping-in/out KV caches and LoRAs, to reduce cold-start overheads and increase the inference performance.

% \shi{Para.9: To address above issues, we propose Logic-Lora, which includes a logic-aware cache manager and a two-stage cache block scheduler. The cache manager captures the logical relationship between kv and lora through a tree structure, and places Loras in the second layer of the tree to ensure their logical relationship. Based on this tree, we insert new blocks through prefix matching and eliminate blocks from leaf nodes to avoid invalid blocks.The cache block scheduler first ensures the minmum number of the Loras through the xxxxxx model to increase the supported throughput. Afterwards, taking into account the recent access time, frequency, and time overhead of swapping in/out, the cost of swap-in/out for cache bock is defined as the expected value of xxxxxx, to find the optimal priority for swap-in/out.}
We therefore propose \textbf{Logic-LoRA}, a LLM cache management system for the Multi-LoRA inference. It consists of a \textit{logic-aware cache manager} and a \textit{two-stage cache swapper}.
The cache manager introduces a \textit{logic tree} to construct logic dependencies between KV caches and LoRAs, where nodes are KV caches or LoRAs and edges are their dependencies. 
To maintain the logic dependencies, LoRAs or KV caches are inserted or eliminated from leaves to keep the tree connected.
% The block swapper decides the swapped-in or swapped-out LoRAs or KV caches into or out of HBM when the HBM is idle and busy, respectively. 
After each fixed monitor interval, the cache swapper first loads the minimum required number of LoRAs into HBM to ensure the supported peak throughput.
Then, it decides the pre swapping-in/out LoRAs or KV caches based on a cost model when the HBM is idle and busy, respectively. This model considers the metrics of recent access time, frequency, and swap-in/swap-out overheads, and define the cost as the expected decrease/increase in the TTFT for future queries.


% \shi{This paper makes three major contributions.}
% \begin{itemize}
%     \item \shi{Characterization of existing multi-tenant lora and kv management strategies. These analysis guides us to perceive the relationship between KV and Lora when managing, and to comprehensively consider xxx when swap-in/out.}
%     \item \shi{A of KV and LORA managers based on tree structure xxx. The manager maintains two types of relationships by placing them in a tree structure and appropriate lora positions on the second layer, avoiding the occupation of invalid blocks in HBM.}
%     \item \shi{Two-stage cache block scheduler to xxx. The scheduler first satisfies the throughput by setting the minimum required number of Lora, and then comprehensively considers xxx, xxx, and xxx to form a cost mode, to determine the optimal swap-in/out cache block.}
% \end{itemize} 
This paper makes three major contributions.
\begin{itemize}
    \item \textbf{Investigating the cache management of LoRAs and KVs for the Multi-LoRA inference.} The analysis motivates us to maintain the logic dependencies between LoRAs and KV caches during inference, and fully considers performance metrics for their swapping-in/out.
    \item \textbf{A cache manger to maintain the logic dependencies between LoRAs and KV caches.} The manager adopts the logic tree to construct the relationships, and inserts or eliminates nodes from the leaves. It maintains the logic dependencies and thus ensures the HBM fully utilized.
    \item \textbf{A cache swapper to pre swap-in/out appropriate LoRAs or KV caches.} The swapper decides the pre swapped-in/out cache blocks based on a cost model, which fully considers relevant performance metrics. It avoids the cold-start overhead during the inference.
\end{itemize}

% \shi{We have evaluated Logic-LoRA on xxx. Evalaution results show xxx.}
We have evaluated Logic-LoRA with Llama-7B/13B/34B models~\cite{touvron2023llama} on eight Atlas 300I NPUs~\cite{xx} under two typical scenarios (chat robot~\cite{luo2024arena,chiang2024chatbot} and multilingual translation~\cite{zhang2020improving}). Experimental results show that Logic-LoRA reduces the TTFT and TPOT by 63.4\% and 40.1\%, respectively, compared to state-of-the-art Multi-LoRA inference systems.


%第一段: LLM和KV cache, HBM和host memory联合使用, 预先加载有收益
%第二段: Lora技术 multi-tenant lora, lora预先hbm加载也可以加速, 这种场景下更困难
%第三段: 需要一个流程图1, multi-tenant lora请求的推理流程, 体现出需要把历史kv以及lora混合cache到hbm中进行管理(标明第一步), lora和历史kv本质上有一定关系(标明第二步), HBM+host memory有限需要合适的换入换出策略
%第四段: 现有的工作静态分割,将hbm固定分给kv和lora; 或者统一内存管理,但没有逻辑关系, 使用简单的LRU进行换入换出block，但是目前的工作都是在TTFT和TPOT等指标上很inefficient,主要原因来源于3个方面
%第五段: 对于第一个原因,静态的hbm分配在各种动态场景下适配性差,一个固定的静态分配往往只适用于一种lora分布场景,lora num/分布/负载量
%第六段: 对于第二个原因,即使统一管理,忽略他们之间的逻辑关系使得内存中存在“invalid block”和“low cache hit rate”, 用图1讲明是什么invalid block, 给一个low cache hit rate的数据
%第七段: 对于第三个原因,合适的预换入\预换出策略是有必要的, 简单的基于LRU策略在multi-lora场景中不work了,因为我们发现需要优先满足lora的数量需求避免冷启动,同时需要考虑更多负载的因素,比如lora频率\换出lora/kv块需要的时间等因素。我们发现LRU决策需要换出的块很多在频率上很高等例子
%第八段: 一个直观的解决方式是在hbm中统一管理KV和Lora,感知kv和lora之间的逻辑关系,并综合谨慎的决策换入换出的cache block。然而，需要利用合适的cache管理结构来维护kv和lora之间的关系，使能在动态场景下具有逻辑指导性地换入/换出cache block。此外，需要定义代价模型来综合各种指标评估调度cache block出入HBM的优先级。
%第九段: 为了解决以上问题，我们提出了Logic-Lora，包含一个logic-aware cache manager和一个two-strage cache block scheduler。cache manager通过树状结构捕获了kv和lora之前的逻辑关系，并将lora放在数中的第二层保证他们的逻辑关系。基于这棵树，我们通过前缀匹配插入新的block，并从leaf node淘汰block以避免invalid block问题。cache block scheduler首先通过xxx模型保证了lora数量下限，以保证所支持的吞吐。之后综合考虑最近访问时间、频率和换入\换出开销，将cache bock的换入\换出cost定义为xxxxxx的期望，以找到最佳的换入/换出优先级。
%第10段: 文章的贡献如下: 
%1) 对于现有multi-tenant lora和kv管理策略的characteriction。这些分析指导我们指导我们需要管理时需要感知kv和lora之间的关系，并在换入换出时综合考虑xxx
%2) 基于树状结果的kv和lora管理器设计。该管理器通过树状结构及恰当的lora位置放置在第二层维护了两种关系，避免了hbm的无效block占用。
%3) 两阶段cache block scheduler设计。该调度器通过满足lora下限满足了吞吐，并将xxx，xxx和xxx综合考虑如cost mode来决策最佳的换入/换出cache block。
%第11段: 我们在xxx环境中evaluate了logic-lora，实验结果表明xxx。





%第一段multi-lora， 用kv cache缓存很多信息
%LRU部分的reason：我们把lora更多放在里面会更好，应该说做到什么行，但是现有lRu做不到
%multi-lora更多的应用场景在intro，personal agent
%说动态性的问题

==> Sections/moti.tex <==
\section{Background and Motivation}
In this section, we first introduce the background of Multi-LoRA serving with caching, and then investigate the inefficiency of current Multi-LoRA serving systems.

\subsection{Multi-LoRA Serving with Caching}
% Figure~\ref{fig:moti_lora_minimum} shows an example Multi-LoRA inference workflow with KV and LoRA caching.

\quan{This subsection is too long. Be simple and to the point.}
% \textit{Use one figure and less formulas.}

\textbf{Multi-LoRA.} 
% Introduce the theory of LoRA, multi-LoRA, and scenarios for multi-LoRA. Mention the SGMV and unified memory pool of S-LoRA.
% LoRA is a popular parameter-efficient fine-tuning method in specializing pre-trained LLM to a specific task, which can achieve high accuracy with small cost. LoRA add new branch adapters to the original weights and just updates these new adapters when fine-tuning. 
% % Compared to full parameter fine-tuning, LoRA reduces the number of trainable parameters by orders of magnitude while retaining comparable accuracy. 
% During multi-task inference, multi-LoRA inference only requires loading a single fine-tuned model, and dynamically load in the target LoRA weights to additional branch, significantly improving inference efficiency.
LoRA is a popular method for efficiently fine-tuning pre-trained LLMs by adding lightweight adapters to original weights, in which only adapters are updated during fine-tuning~\cite{xx,xx}. For Multi-LoRA inference, the pre-trained model is loaded once, and adapters are dynamically applied based on user queries, enhancing inference efficiency~\cite{xx,xx}.
% in specializing pre-trained LLM to a specific task using a new branch adapters added to the original weights. When fine-tuning, just need to update these new adapters. 
% Compared to full parameter fine-tuning, LoRA reduces the number of trainable parameters by orders of magnitude while retaining comparable accuracy. 
% During Multi-LoRA inference, only a pre-trained model is needed to be loaded and the loRAs are dynamically loaded to additional branch according to user queries's demands, improving inference efficiency.

% When providing multi-LoRA serving, the simplest method is to merge LoRA weights with pre-trained LLM weights before inference based on query's requirements and separating them afterward. However, this process introduces substantial overhead and prevents different LoRA requests from being inferred in the same batch, making it impossible for large-scale Multi-LoRA services. 


% As shown in Figure~\ref{fig:moti_multi_lora}, 
The common approach for Multi-LoRA serving uses an inference kernel like Segmented Gather Matrix-Vector multiplication (SGMV)~\cite{xx,xx}, allowing different queries and their LoRAs to be processed in a single batch.
This method ensures the correctness while enhancing the inference efficiency and throughput through batch processing.
% Moreover, to save HBM space, LoRAs are usually offloaded to host memory and swapped-in/out on-demand~\cite{xx,xx}.
% For instance, S-LoRA~\cite{xx} uses a unified paging design to store LoRAs and KV cache in a shared memory pool of HBM, which reduces the fragmentation and enhances the HBM utilization efficiency.
% Because the sizes of LoRA weights and KV cache are aligned at each layer, they can effectively fill the entire memory pool with minimal memory fragmentation, thus enhancing the system’s memory utilization efficiency.

\textbf{Caching of KVs or LoRAs.} 
% Introduce the KV prefix matching, and logic dependencies with LoRAs
Most LLMs use a decoder-only transformer to predict the next token with KV caches computed from previous tokens~\cite{xx,xx}. Thus, when a query matches an existing prefix, the system can reuse the stored KV cache, reducing HBM usage and eliminating redundant computations, such as multi-turn dialogues~\cite{xx,xx}. Compared to destroying all KV caches after the query returns, history KV caches can be maintained in HBM to maximize reuse.
% The inference system always retains history KV cache in HBM. To ensure correct matching, the inference system need to maintain the logical relationships between history KV cache using data structures such as linked lists and hash tables. For multi-LoRA inference, since LoRA branch contributes to the generation of KV cache, KV caches corresponding to different LoRA weights cannot be shared and must be stored and managed separately. Consequently, the LLM inference system also needs to add new LoRA weight label to the history KV cache. Similar to the swap in/out strategies mentioned earlier for LoRA weights, history KV cache can also be offloaded to main memory to free HBM resources for inference. Howerver, swap in needed history KV cache and LoRA on demand can lead to cold start overhead, which directly impacts performance metrics such as TTFT. To minimize this overhead, the inference system needs to pre-fetch "hot" history KV cache and LoRA to HBM. 
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/background_multi_lora-new-3.pdf}
    \caption{An example of the Multi-LoRA inference workflow with the caching of KVs and LoRAs.} 
    \label{fig:moti_multi_lora}
    \vspace{-3mm}
\end{figure}

As shown in Figure~\ref{fig:moti_multi_lora}, KV caches for different LoRAs have to be stored separately due to additional LoRA branch which involves in the computation of KV cache~\cite{xx,xx}.
% and current systems~\cite{xx,xx} generally add LoRA labels to each history KV cache. 
The separate storage exacerbates the contention of limited HBM space, and thus the KV caches and LoRAs are usually offloaded to main memory and swapped-in/out on-demand~\cite{xx,xx}.
However, this can cause cold-starts when swapping them back to the HBM, affecting performance metrics like TTFT and TPOT.
To reduce this overhead, the inference system needs to pre-cache the ``hot'' history KV caches and LoRAs onto the HBM.

\quan{You also mention several overhead here? Figure 2 seems a little bit complex. If you mention the three overheads, please better present them. }
\textbf{Multi-LoRA Serving.} 
% Different from Figure-1, introduce the serving of multi-lora queries, what will happen.
% Explain the goal we want to optimze (TTFT/TPOT), we need to reduce cold start latency of loras and KVs, so needing better pre-cache strategies.
As shown in Figure~\ref{fig:moti_multi_lora}, the processing workflow of a newly-arrived Query-2 is as follows: 
\ding{172} Since LoRA-1 is not in HBM, its dependent KV1-1 and KV1-3 in HBM cannot be matched by queries due to the \textit{usage dependencies}.
These invalid KVs cause HBM space to be insufficient, thus Query-2 needs to wait for them to be swapped-out, leading to the queuing time.
\ding{173} Although KV2-1 is in HBM, Query-2 needs to load LoRA-2 first due to the \textit{usage dependencies} between LoRAs and KVs, resulting in the LoRA cold-start overhead.
% During the cold-start period KV2-1 is invalid but occupies the HBM, preventing other queries from loading their required KVs or LoRAs into the HBM.
\ding{174} Query-2 waits for KV2-2 to be swapped in, adding KV cold-start overhead. 
\ding{175} Query-2 is processed with other queries in batch using the SGMV kernel, generating the new token and KV cache.

% \SJC{The above para needs to describe the serving of multiple queries, not a single one. Moreover, present the ``logic dependency'' during the workflow.}

Therefore, the overheads that affecting the inference performance (TTFT and TPOT) includes the queuing time (\ding{172}), as well as the LoRA or KV cold-start time (\ding{173}-\ding{174}).
These overheads are caused by the unawareness of usage dependencies between KVs and LoRAs and inappropriate swap-in/out of KVs and LoRAs between the HBM and main memory.
% The queuing time is mainly caused by the invalid KV caches under \textcolor{red}{the unawareness of logic dependencies between KVs and LoRAs??}. Moreover, the pre-caching strategy to properly decide the swapping-in/out of KVs and LoRAs can reduce their cold-start time. 

% The key metrics TTFT is mainly affected by the above parts. 
% \textcolor{red}{By designing effective LoRA and KV cache pre-caching strategies under the maintainence of the logic dependencies, the cold-start overhead of LoRAs and KV caches can be directly reduced.} This can enhance inference efficiency and throughput, reflecting on TTFT and TPOT.

% For the key metrics of LLM services, TTFT, it encompasses: 1. Queuing time after the request arrives. 2. Cold-start overhead of LoRA weights. 3. Cold-start overhead of corresponding history KV cache. 4. Inference time of prefill phase. 5. Communication delays, among others. By implementing effective LoRA and KV cache prefetching strategies, the cold-start overhead of LoRA and KV cache can be directly reduced, thereby decreasing TTFT. This also enhances overall efficiency and throughput, optimizing metrics such as TPOT.

\subsection{Low Multi-LoRA Serving Performance}
%baselines 
This subsection investigates the query inference performance of current Multi-LoRA serving systems.

\quan{Besides of vLLM, any other prior related work?}

% We choose the vLLM~\cite{xx} as the representative serving system, whose new version supports to manage both the KV caches and LoRAs in the HBM.
Some current works have proposed to cache both LoRAs and history KVs~\cite{xx,xx}, and we choose the most mature work vLLM~\cite{xx} as the representative baseline in this subsection. vLLM allocates the fixed HBM space for LoRAs and KV caches separately, and utilizes the LRU to swap-in/out LoRAs or KV caches in their individual HBM area.
The vLLM also requires a predefined allocation ratio of the HBM space for the LoRA, and we set it to 0.3 where 100 LoRAs can be fully loaded in the HBM. Referring to the latest version vLLM, we set the memory block size to 32. 

%datasets, models, and hardwards
We utilize the LMSYS-33k~\cite{xx} dataset to construct outputs of the queries for the chatbot scenario. The LMSYS-33k contains 33,000 human dialogue samples during 3 months from 20 different LLMs like GPT-4~\cite{xx} and Claude-v1~\cite{xx}.
Moreover, we use the Llama-7B as the base model. 
We conduct the experiments on one Atlas 300I NPU~\cite{xx}, and Table~\ref{table:config} summarizes the hardware and software configurations.

\quan{We should mention why we design the experiment in this way, what is the purpose.}

%detailed experiments
According to production traces~\cite{xx,xx,xx}, the distribution of queries accessing different LoRAs is dynamic. Thus, we construct experiment scenarios with different numbers of LoRAs and different LoRA distributions, as well as various sending rate. In the experiments, we vary the number of LoRAs in the set of \{50,100\} and randomly set their rank to 32 or 64. The distribution of LoRAs used in queries is constructed based on the Gaussian distribution~\cite{xx}, with the standard deviation is in the set of \{0.05,0.1,0.3\}. The query sending rate is adjusted in the set of \{0.6,0.9,1.2\}. 


\begin{table}
    \small
    \setlength\tabcolsep{2pt}
    \caption{Experiment specifications}
    \centering  
    \begin{tabular}{c|c}
      \hline
        & \textbf{Specifications} \\
      \hline
      \multirow{3}*{\textbf{Hardware}}
       & Kunpeng 920 CPU (192 cores), 256GB memory \\
       & 8 $\times$ Atlas 300I NPUs with each of 64GB HBM\\
       & PCIe $\times$ 16 Gen3.0, HCCS 56GB/s\\
       \hline
       \multirow{3}*{\textbf{Software}} & OpenEuler 24.03 LTS\\
       % vLLM-0.4.3\textcolor{red}{Newest version?}
       & Llama-7B, Llama-13B, and Llama-34B\\
       & LMSYS-33K~\cite{xx} and Microsoft Azure Function~\cite{xxx}\\
        \hline 
    \end{tabular}
    \label{table:config} 
    \vspace{-3mm}
  \end{table}
\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{Figures/intro+moti/vllm_ttft.pdf}
    % \includegraphics[width=.9\linewidth]{Figures/intro+moti/vllm_tpot.pdf}
    \caption{The TTFT of vLLM-default and vLLM-Oracle under different scenarios. \SJC{Use 18 scenarios, use truncated graph, x-label needs to be same to Figure4.}}
    \label{fig:moti_vllm}
    \vspace{-3mm}
\end{figure}

\quan{We should explain the $x$-axis. The baselines, etc.}

%results
Combining all the above experiment settings, a total of 18 scenarios are obtained. Figure~\ref{fig:moti_vllm} shows the TTFT of vLLM-Default and vLLM-Oracle under these scenarios.
vLLM-Oracle represents the results with the best HBM allocation ratio of LoRAs, which are achieved by profiled in the range from 0.1 to 0.9, and the vLLM-Default is set as 0.3 as we mentioned before.
% \textcolor{red}{(all xxx LoRAs can be loaded into HBM )}, and more HBM for LoRAs is as waste
The x-axis represents the experiment settings, e.g., (50,0.1,0.6) represents the LoRA number, standard deviation, and sending rate equal to 50, 0.1, and 0.6, respectively.
The red line with the right y-axis shows the HBM allocation ratio of the vLLM-Oracle. 

We can observe that the vLLM needs different LoRA allocation rate to achieve the best TTFT under different scenarios.
The maximum HBM allocation ratio is 0.3 as all 100 LoRAs can be loaded into the HBM under this ratio.
As statistics, the vLLM-Default increases the TTFT by 96.1\% on average compared to vLLM-Oracle.
Since the increase of TTFT, vLLM-Default's TPOT is also increased by 16.4\% than vLLM-Oracle.
The above results prove that the static HBM allocation of vLLM cannot adapt to all dynamic scenarios for the Multi-LoRA serving.
% \quan{We need to give some quantitative data.} We also HBM usage of vLLM-default is 13.4\% less than vLLM-Oracle.
% \SJC{Why lots of bars are directly 500?}

\subsection{Diving into In-depth Reasons\label{moti-2}}
Even if static HBM allocation ratio under dynamic scenarios is determined from ideal profiling, the management of LoRAs and KV caches is also inefficient due to two in-depth reasons, including: 1) \textit{low HBM utilization without intra-LoRA usage dependencies} and 2) \textit{inappropriate swap-in/out for KVs and LoRAs under inter-LoRA dynamics}.

\subsubsection{Low HBM Utilization without Intra-LoRA Usage Dependencies}
% No matter statically partition or unified manage the HBM, 
Current works~\cite{xx,xx,xx} did not and maintain the intra-LoRA usage dependencies between LoRAs and KVs in the HBM. We use the vLLM-oracle in this subsection for analysis.

\begin{figure}
    \centering
    % \includegraphics[width=.9\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-invalidrate.pdf}
    % \includegraphics[width=.9\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti_hitrate.pdf}
    \includegraphics[width=.9\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-oracle_hit_valid.pdf}
    \caption{The invalid KV caches and cache hit rate for the vLLM-Oracle under various scenarios.}
    \label{fig:moti_logic}
    \vspace{-3mm}
\end{figure}

Figure~\ref{fig:moti_logic} shows the invalid KV caches and cache hit rate for the vLLM-Oracle under various scenarios. 
We can first observe that they are considerable invalid KV caches in the HBM, with an average value of 48.1\%. 
The large mount of invalid KV caches result in low utilization efficiency of HBM, preventing the other LoRAs or KV caches being loaded in the HBM. 
Thus, from this figure, we can also observe that cache hit rate under different scenarios in not high, with an average value of 69.9\%.
In Section~\ref{eval}, when being aware of the logic dependencies and maintain them in the HBM, \sysname{} can have no invalid KV caches and can achieve a cache hit rate of 81.8\% on average.

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-example-new-2.pdf}
    \caption{Examples of serving two queries under: (a) without usage dependencies, and (b) maintaining usage dependencies.}
    \label{fig:moti_example}
    \vspace{-3mm}
\end{figure}

% To better understand how logic unawareness causes HBM under-utilization, we take an example of two queries in Figure~\ref{fig:moti_example}.
% When logic unawareness in (a), since the LoRA-1 needs cold-start, three KV caches cannot be matched but take up the HBM space, making them be ``invalid''. 
% After LoRA-1's cold-start, Q1 conducts the subsequent inference.
% Meanwhile, Q2 first matches the LoRA-2 and has to wait Q1 to finish, before matching LoRA-2 and subsequent KVs, resulting in a long waiting time. 
% The average execution time of the two queries is 11 time-slots.
% When we maintain the logic dependencies in (b), the three KVs will be not in the HBM and the required KV caches can be pre-cached.
% In this way, Q2 can finish the inference without waiting.
% Despite Q1 needs more cold-start time, but the average execution time reduces to 8 time-slots.
To better understand how usage unawareness causes HBM under-utilization, we take an example of two queries in Figure~\ref{fig:moti_example}. Suppose two queries (Q1 and Q2) to be executed. Without the usage dependencies in (a), since the LoRA-2 needs cold-start, the KV2-1 cannot be matched but occupy the HBM space, making it be ``invalid''. Although Q1 successfully matches LoRA-1, due to the lack of space, it must queue to wait for KV2-1 to be swapped out, then Q1 can swap in required history KV cache and execute successfully. After Q1 finishing, Q2 needs to re-swap in KV2-1 again to perform inference. This causes redundant swap-in/out, and the queuing overhead is increased. 
By contrast, when maintaining the usage dependencies as (b), Q1 directly matches LoRA-1 with its required history KV cache KV1-1 and executes the inference immediately without any queuing. Then, Q2 swaps-in/out and executes inference afterward. 
In this way, the redundant swap-in/out is eliminated, and the total running time of both Q1 and Q2 both reduces.

% \textcolor{red}{Above content needs to be updated.}

\subsubsection{Inappropriate Swap-in/out for KVs and LoRAs under Inter-LoRA Dynamics}
Previous works~\cite{xx,xx,xx} separately managed the LoRAs and KVs in individual HBM area, and adopted simple caching strategies like the Least-Recent-Used (LRU) for swap-in/out.
These works cannot dynamically balance the HBM usage for LoRAs and KVs when the loads of different LoRAs change.
% For unified managing the swap-in/out of LoRAs and KVs in the HBM, we mainly have two observations to improve the inference performance.
% which cannot balance the HBM usage for them when loads 
% adopted the LRU strategy for swapping-in/out the KVs and LoRAs. 
% However, this strategy can lead to inappropriate pre-caching. 

\begin{figure}
    \centering
    % \includegraphics[width=0.45\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti_need_lora_1.pdf}
    % \includegraphics[width=0.45\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti_need_lora_2.pdf}
    \includegraphics[width=.8\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-ttftwithlora.pdf}
    \caption{The TTFT of vLLM under different HBM allocation ratios for LoRAs. \SJC{use truncated graph, rate->ratio, mark the ``target ratio'' using red circles in this figure.}}
    \label{fig:moti_lora_minimum} 
    \vspace{-3mm}
\end{figure}

Figure~\ref{fig:moti_lora_minimum} shows the TTFT of vLLM under different HBM allocation ratios for LoRAs at the scenarios (50,0.1,1.2) and (100,0.1,1.2), respectively.
% The throughput is calculated by the number of queries completed per minute (QPM).
We can observe that the TTFT declines significantly after achieving at a target ratio, and the target ratio is increased when the LoRA number changes from 50 to 100.
Above results prove that 
% the insufficient HBM reservation for LoRAs can greatly harms the TTFT, and the HBM reservation
different HBM space needs to be reserved to cache LoRAs to greatly reduce the TTFT under dynamic scenarios, while a fixed HBM allocation cannot adjust the reservation accordingly.
% \textcolor{red}{Maybe revise the above text.}

\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-frequency.pdf}
    \includegraphics[width=0.32\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-swapcost.pdf}
    \includegraphics[width=0.32\linewidth]{ATC2025-Logic-LoRA/Figures/intro+moti/moti-recomputecost.pdf}
    \caption{The relationships between the visited frequency, swap costs, and re-compute costs to last visited time (LRU) of the KV caches or LoRAs.}
    \label{fig:moti_LRU}
    \vspace{-3mm}
\end{figure}

Moreover, to swap-in/out appropriate LoRAs and KVs under dynamic loads of different LoRAs, it is fine to directly access their effect to TTFT for decisions.
The TTFT is strongly related to metrics of the visited frequency, last visited time, swap cost, and recompute cost~\cite{xx,xx,xx}.
Thus, for all set of experiments, we collect all above metrics and rank them.
Figure~\ref{fig:moti_LRU} shows the ranking relationships among these metrics. We can observe that these has little correlations.
As these metrics are all useful in optimizing the TTFT when conducting swap-in/out, thus previous simple caching strategies like LRU cannot make appropriate decisions.

%2.1 figure-2不要  写工作原理，少写问题
%2.2 换成3个benchmark的随时间轴，vllm的TTFT变化
%2.3.1： figure-4不要，写统计数据；figure-5全栏详细描述，4t这些东西不要
%2.3.2：figure-6不要了，从2.2中去找去说明；我们说成需要cost model来动态balance KV 和lora

%流程上有这些影响因素



